Compositionally Generalizable 3D Structure Prediction

Single-image 3D shape reconstruction is an important and long-standing problem in computer vision. A plethora of existing works is constantly pushing the state-of-the-art performance in the deep learning era. However, there remains a much more difficult and under-explored issue on how to generalize the learned skills over unseen object categories that have very different shape geometry distributions. In this paper, we bring in the concept of compositional generalizability and propose a novel framework that could better generalize to these unseen categories. We factorize the 3D shape reconstruction problem into proper sub-problems, each of which is tackled by a carefully designed neural sub-module with generalizability concerns. The intuition behind our formulation is that object parts (slates and cylindrical parts), their relationships (adjacency and translation symmetry), and shape substructures (T-junctions and a symmetric group of parts) are mostly shared across object categories, even though object geometries may look very different (e.g. chairs and cabinets). Experiments on PartNet show that we achieve superior performance than state-of-the-art. This validates our problem factorization and network designs.

==> tex/method_arxiv.tex <==
\section{Method}
Compared to previous methods, our proposed algorithm is trained only on the chair category and can generalize to unseen categories, such as bed, cabinet, and table. The key observation is that shapes across categories share similar parts and local part relationships, supporting compositional generalizability.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{./fig/figure_overview}
    \caption{Our single-view 3D structure prediction pipeline. To extract the 3D structure from a single input image, we go through the following pipeline: (a) we apply MaskRCNN to extract the part instance masks; (b) we identify parallelism for part pairs, form parallel part groups, and predict the shared edge directions for each group; (c) we identify translational symmetry within part pairs, group parts with equal size, and predict the shared edge length; (d) we predict the connectivity for part pairs and extract a connectivity-based part tree; (e) we predict the relative position between adjacent parts and assemble the whole shape while traversing the part tree. We heavily use part masks as module inputs to induce a focus on local regions following the isolation principle. And we rely on pairwise relationships from (b)-(e) which reflects the relativity principle.}
    \label{fig:overview}
    \vspace{-4mm}
\end{figure*}

%\subsection{Overview}
In our pipeline, we first learn to predict part masks using MaskRCNN~\cite{he2017mask}, a well-established object instance segmentation approach (Sec~\ref{sec:method:part_seg}). 
% Next, we learn to predict prominent relationships between parts,
% which will be used for the estimation of part principal axes directions, part scale, and the relative position between parts. 
% We defer the precise definition of these relationships as well as the corresponding discussions into later sections when these relationships are first used.
In Sec~\ref{sec:method:part_dir_pred} and Sec~\ref{sec:method:part_scale_pred}, we introduce how to predict the direction and size of the oriented bounding cuboid for each part. Finally, in Sec~\ref{sec:method:part_assembly}, we introduce how to assemble the predicted cuboids into a complete shape.

\subsection{Part Instance Segmentation} 
\label{sec:method:part_seg}
The first step of our pipeline is to obtain the mask of each part in the input image. The goal of this step is exactly the same as the classical instance-level object segmentation problem. Due to the popularity of research into instance-level segmentation, we do not treat this step as the focus of our work. Instead, we borrow existing methods to obtain the part masks. Particularly,  we choose the well-established MaskRCNN~\cite{he2017mask} and train it using the finest part masks rendered from PartNet. Please refer to Sec~\ref{sec:supp_part_instance_seg} in the supplementary material for details.
%As an alternative, we also evaluate with human annotated part masks following the part definition in PartNet. 

It is reasonable to expect that learning-based approaches can transfer across categories for primitive-level part detection and segmentation.
In our daily experience, though objects from different categories vary a lot in geometry, their part appearance usually share a lot similarity, especially for man-made objects. Such part-level similarity could be attributed to many factors, such as to fulfill affordance constraints (thin bars are suitable for grasping), manufacturing constraints (planes are easier to machining), and functionality constraints (wheels enable laborless movement). Besides, primitive parts tend to be made by the same material and painted with homogeneous textures, and their local geometrical patterns are usually simple (\eg, uniform curvature). Such uniformity would yield appearance patterns easily captured by Convolutional Neural Networks. According to our experiment in Sec~\ref{sec:exp:ablation}, MaskRCNN trained on chairs only achieves high performance on novel categories such as bed, cabinet, and table. 
  
\subsection{Part Cuboid Edge Direction Prediction} 
\label{sec:method:part_dir_pred}

To represent the orientation of each part cuboid, we leverage the principal axes directions, which we refer to as edge directions. Provided with an image and a binary mask of each part, we design a neural network to estimate such edge directions. Specifically, we encode edge directions with a rotation matrix where each unit vector in a row corresponds to one edge and the network simply needs to regress the rotation matrix.
Notice the definition of such rotation matrices suffers from ambiguities since each of the rotations falls into an equivalent class containing 24 elements (considering the permutation of axes and flipping of axes directions). Naively supervising the learning process with ambiguous and inconsistent ground truth would hinder the network training seriously as illustrated in Sec~\ref{sec:exp:ablation}.
%However, due to the symmetry of the cuboid, there exist a set of equivalent rotations (at least 4 and at most 24) corresponding to the same geometry.
%It is not trivial to define a canonical representative of equivalent rotations across instances, while learning naively with ambiguous and potentially inconsistent supervision would hinder the network training as illustrated in Sec~\ref{sec:exp:ablation}.
%To get rid of the rotation ambiguity, we expect 
%we only expect that the three coordinate axes induced by the predicted rotation match those induced by the ground truth in an orderless fashion.
%Note that the coordinate axes induced by rotation correspond to the edge directions of cuboid.
% \jigu{Fig~\ref{fig:edge_dir_pred} illustrates the definition of edge direction.}

We summarize the innovations of our design here and include details in Sec~\ref{sec:supp_edge_direction} of the supplementary material. To resolve the rotation ambiguity, instead of directly supervising the rotation, we evaluate its effect on a unit cube and define a proxy loss using the cube geometry.
% Focusing on estimating edge directions, we apply a proxy loss on a unit cube to supervise the predicted rotation.
To be specific, the geometry of the unit cube is represented by its 8 vertices, denoted by $P_{\text{cube}} \in \mathbb{R}^{8 \times 3}$.
The ground truth and predicted rotations are denoted by $R$ and $\hat{R}$.
%, where $\hat{R}$ is parameterized by quaternion $\hat{q}$.
The objective is to minimize a geometric loss $L_1=D(P_{\text{cube}}\hat{R}^T, P_{\text{cube}}R^T)$ between the rotated unit cube $P_{\text{cube}}\hat{R}^T$ and the ground truth unit cube $P_{\text{cube}}R^T$, where $D(\cdot, \cdot)$ is a distance measurement which could be either Chamfer Distance or Earth Mover's Distance.
% We use $D(P_{cube}\hat{R}^T, P_{cube}R^T)$ to, where $D$ is a distance metric, \eg, Chamfer Distance or Earth Mover's Distance.
% Considering the equivalent class of rotation $\{R_i\}$, the loss is designed as $L_1=\min_{i}{D(P_{cube}\hat{R}^T, P_{cube}R_i^T)}$.
% We denote it by \emph{Min-of-N Loss}.
We supervise a ResNet to predict $\hat{R}$.
%the quaternion $\hat{q}$ which paramterizes 
%$\hat{R}$, given the concatenation of image and mask as input.

% However, \emph{Min-of-N Loss} is vulnerable to local minimum caused by initialization.
However, combining the geometric loss with a single-branch ResNet fails to solve the problem nicely in practice. This is mainly due to its vulnerability to local minimum caused by the network initialization.
To ease the optimization, we introduce \emph{Mixture of Experts Network} (MOE).
Concretely, given the features extracted by the backbone, multiple branches (a.k.a. ``experts'') are applied to predict multiple 
rotations $\{\hat{R}_j\}$
% quaternions $\{q_j\}$, 
as well as probabilities $\{\hat{q}_j\}$ to select certain branches.
The loss is then updated as $L_2=\min_{j}D(P_{\text{cube}}\hat{R_j}^T, P_{\text{cube}}R^T)$.
%$L_2=\min_{j} L_1(\hat{R}_j) = \min_{j}\min_{i}{D(P_{cube}\hat{R}_j^T, P_{cube}R_i^T)}$.
Besides, we also maximize the log likelihood of the predictions under a mixture of Laplacian distributions, which is formulated as 
$L_3=\log \sum_{j} \hat{q}_j \frac{1}{2b} e^{-\frac{D(P_{\text{cube}}\hat{R_j}^T, P_{\text{cube}}R^T)}{b}}$.
The overall training loss is $L_2+\lambda L_3$.
During inference, we select the branch with the maximum probability $\hat{q}_j$ to predict $\hat{R}_j$.


Instead of processing each part individually, we group parallel parts who share edge directions. In this case, we only need to predict the shared edge direction for each group. This allows us to leverage the complementary information among parallel parts and resolve ambiguities potentially caused by occlusion or perspective projection.
% it might be helpful to utilize the parallelism, so that the estimation of each part can benefit from complementary information of other parallel parts.
% Different part groups can be formed, so that parts in the same group are parallel to each other, and their rotations should be unified.
To this end, we first train a ResNet that consumes the concatenation of an image and a pair of part masks to classify whether the pair of parts are parallel. For the details of part relationship prediction, please refer to Sec~\ref{sec:supp_part_relation} in the supplementary material.
The groundtruth labels are generated by a heuristic algorithm, described in the supplementary.
% During inference, a pair of parts is considered parallel if the classification score is above a predefined threshold.
During inference, we cluster parts into groups so that pairs of parts in each group are all classified as parallel.
To predict the shared edge directions for each group, we first employ a ResNet to extract the features of individual parts, and then aggregate them through max-pooling. The aggregated feature is finally passed through a regression head to output edge directions.
% To predict the rotation of a group of parallel parts, we employ a shared ResNet to extract the feature of each part, and use a max-pooling layer to aggregate them.
% The final rotation of the group is predicted based on the aggregated feature, supervised by the loss discussed above.


\subsection{Part Cuboid Edge Length Prediction} 
\label{sec:method:part_scale_pred}


The goal of this step is to predict the size of all the parts. This step takes three inputs: the image, a binary mask of each part, and a set of three unit vectors denoting the edge directions of the part cuboid. It should output the edge length along each edge direction for all the parts. We summarize our design here and include details in Sec~\ref{sec:supp_edge_length} of the supplementary material.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{./fig/edge_length_prediction}
    \caption{Part cuboid edge length prediction. We use this network to predict shared edge length for each group of translational symmetric parts. We first stack the input reference image and the mask image of each part.We use a shared ResNet to extract per-part feature, which are then max-pooled to generate a group feature. We combine the group feature with predicted edge directions from Sec~\ref{sec:method:part_dir_pred} to further estimate the edge length.}
    \label{fig:edge_length_pred}
    \vspace{-4mm}
\end{figure}

Similar to Sec~\ref{sec:method:part_dir_pred}, we believe that predicting part size in groups may help to improve prediction performance. Here, we form part groups by considering translational symmetry, yet our idea may be extended to leverage more symmetry types. Specifically, we group all parts into several clusters, so that parts in the same cluster can be translated to each other. The clustering scheme will allow us to predict a unified size for all the member parts in each cluster. Predicting part sizes in clusters brings at least three advantages: (1) Compared with predicting part sizes individually, we have more evidences from the input. Particularly, it significantly helps to reduce the ambiguity of object sizes under perspective projection; (2) Some parts may not be fully visible due to occlusions, and predicting their sizes individually is very difficult; (3) Having a unified size for translational symmetric parts is visually much more pleasing for humans.

At test time, we train a translational symmetry classifier to help form clusters. The classifier is a ResNet that consumes an image and a pair of part masks stacked together as the input. This ResNet is trained supervisedly to tell whether the two parts highlighted by the input masks follow translational symmetry. Then, we build clusters of parts so that classification scores between any pair of parts in the same cluster are above a predefined threshold. We find that this classifier is transferable across categories by our experiments in Sec~\ref{sec:exp:ablation}.

We are ready to predict the part size for each cluster of parts. Our architecture is illustrated in Fig.~\ref{fig:edge_length_pred}. We first use ResNet with shared weights to predict the features for each part in a cluster independently. Note that the input to each branch is the image and the mask of a single part. The mask induces the network to focus on the masked region, and since we only couple a single part mask with the image, it forms a low-order prediction task. We then use a max pooling layer to aggregate features of each individual part. No additional interaction across parts are allowed, which reduces the risk of making predictions by high-order potentials of parts. Finally, the aggregated feature is duplicated three times and coupled with each of the predicted edge directions from the edge direction prediction module (Sec~\ref{sec:method:part_dir_pred}). The purpose is to query the edge length along each direction.  This edge length prediction network is learned supervisedly by mean square loss.





\subsection{Part Cuboid Assembly} 
\label{sec:method:part_assembly}

% \subsubsection{Image features}
% To estimate geometry primitives for each part, we need to extract image features from image and part masks. We use a ResNet18 as the backbone module to compute a 2D feature map $f_i$. Our input image and mask dimensions are $256 \times 256$. We then embed the feature map $f_i$ into global feature $x^g$ with one layer convolution with stride equal to 2 and one average pooling layer with kernel equal to 4.
% 
% For unary part estimation, we concatenate the image and part mask in the RGB channels. The input feature channel of ResNet18 is set to be 4. Similarly, for binary part prediction, we concatenate the image and two part-masks and the input channels of ResNet18 are set to be 5.
%  
Having computed the part mask, edge directions, and size of individual parts, this module learns to assemble them into a whole shape. Following the isolation principle, we restrict the reasoning process to be only based upon pairwise relationships. To this end, we first build a part tree, whose nodes are parts, and edges indicate the pairs of parts for assembly reasoning. Then, based on the relativity principle, we predict the relative position between each pair of parts in the tree. Finally, we create the whole shape starting from adding the root part with its predicted edge direction and scale. Then we traverse the part tree descendingly and add other parts following their relative position prediction. Please refer to  Sec~\ref{sec:supp_relative_position} of the supplementary material for details.

Our relative position based assembly pipeline is significantly different from most work in the 3D deep learning literature.  Most previous work estimates absolute location in the camera space, the world space, or a canonical object space. However, absolute locations are sensitive to the shape scale as well as the translation along the optical axis, significantly hurting the performance even for the simpler within-category prediction setup. While shape-level canonicalization is often conducted to mitigate the issue in literature, for unknown object categories, any prediction involving the undefined ``canonical object space'' is ill-posed.


% whole shape level understanding is undefined what the canonical space is, and it is unreasonable to assume that we can achieve the a representation robust to scale changes is desired. Here, we design a contact point representation, which we infer the contact point in each primitive frame coordinates and assemble the two parts together based on the fact that the contact point should be the same. In the following, we formulate how to infer the relative location from contact point predictions and give more details of our module to predict the contact point in each primitive frame.

\mypara{Connectivity-based Part Tree.} 
We seek for strong pairwise relationships to assemble parts. In our implementation, we choose the connectivity-based relationship. Our general plan is to first identify spatially contacted pairs of parts, and then predict the relative position between them. We choose this relationship for three reasons: First, parts with contact points are spatially close and impose strong arrangement constraints to each other; Second, when occlusion is absent, assessing whether two parts are in touch is often not too hard from the image space and does not require category-level knowledge; Third, the relationship is quite common. The second and third reasons actually imply good transferability to novel category objects.

We train a connectivity classifier to assess whether a pair of parts touch each other in its original 3D shape. The training is supervised. Based upon the prediction of connectivity scores between all part pairs, we start to form a part tree. First, we build a graph of parts and connect pairs with scores above a threshold. Then, we use a greedy algorithm to build a spanning tree. Specifically, we choose the largest part (by predicted volume) as the root node. Next, we iteratively add more parts by selecting the largest remaining part in the 1-hop neighborhood of the current tree.
Notice when the graph contains multiple connected components, we will simply generate a part tree for each component and form a part forest.

\mypara{Joint-based Relative Position.}
We predict the relative position for selected part pairs in the part tree. The input includes the reference image and the information about each individual part in the pair. The output is the relative position between their part cuboid centers.  

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{./fig/part_assembly}
    \caption{Relative position prediction. Left: Parameterize relative position between part centers (orange and blue spheres) by contact points (green sphere). Right: Network architecture illustration.}
    \label{fig:pos_pred}
    \vspace{-4mm}
\end{figure}

Instead of directly predicting relative center positions, we use a contact point based approach, which incorporates stronger relative position prior. The contact point between touching part pairs must lie within the cuboid of each part. Therefore, we obtain hard constraints over the relative position between part centers. In the following, we formulate how to infer the relative center position from contact point predictions~(read Fig.~\ref{fig:pos_pred} for better understanding): 

\begin{itemize}[leftmargin=+0.1in]
    \item \para{Contact Point.} We use superscript to denote frame and subscript to denote part indices. Given two touching parts $p_1$ and $p_2$, we denote the contact point in a part frame sitting at the center of $p_1$ by $c^1$, and in a different part frame sitting at the center of $p_2$ by $c^2$.\footnote{The orientation of the two frames can be arbitrarily chosen.} We denote the part centers in the world frame as $l^W_1$ and $l^W_2$. Because the contact point is the same, we have the following constraint:
    \begin{equation}
    	l^W_1 + c^1 = l^W_2 + c^2
    \end{equation}
    The relative center location $l^W_{1\rightarrow_2}$ can be inferred as:
    \begin{equation}
    	l^W_{1\rightarrow_2} = l^W_2 - l^W_1 = c^1 - c^2.
    \end{equation}
    Next we discuss how to estimate the contact point $c^i$ in part frame.
    \item \para{Contact Point Estimation.} As the contact should be lying on the part cuboid surface or inside the cuboid, we denote the contact points $c^i$ as a linear interpolation of the cuboid vertices $v_{i, \cdot}$: $c^i = \sum\limits_{j=1}^8 \omega_{i,j} \cdot v_{i,j}$, where $\sum\limits_{j=1}^8 \omega_{i,j} = 1$ and $\omega_{i,j} \geq 0$. 
    We use a neural network to predict $\omega_{i,j}$'s. This network uses a softmax layer to satisfy the above two constraints. Our network consumes a stack containing the reference image and two part mask images and outputs a feature vector. 
    % concatenation of the image and two part masks as the input 
    % to generate a feature vector, and then 
    We pair the feature vector with each vertex position $v_{i,j}$ of the two predicted part cuboids and use another network to predict $\omega_{i,j}$'s. To make the contact point estimation invariant to the ordering of cuboid vertices, the architecture of the second network is similar to the PointNet segmentation network~\cite{qi2017pointnet}. Note that we share some network parameters with other modules. For more details, please refer to Sec~\ref{sec:supp_relative_position} in the supplementary materials. 
\end{itemize}
